Disk Turbulence and Star Formation Regulation in High$-z$ Main Sequence Analogue Galaxies

The gas-phase velocity dispersions in disk galaxies, which trace turbulence in the interstellar medium, are observed to increase with lookback time. However, the mechanisms that set this rise in turbulence are observationally poorly constrained. To address this, we combine kiloparsec-scale ALMA observations of CO(3-2) and CO(4-3) with HST observations of H$\alpha$ to characterize the molecular gas and star formation properties of seven local analogues of main sequence galaxies at $z \sim 1-2$, drawn from the DYNAMO sample. Investigating the ''molecular gas main sequence'' on kpc-scales, we find that galaxies in our sample are more gas-rich than local star-forming galaxies at all disk positions. We measure beam smearing corrected molecular gas velocity dispersions and relate them to the molecular gas and star formation rate surface densities. Despite being relatively nearby ($z \sim 0.1$), DYNAMO galaxies exhibit high velocity dispersions and gas and star formation rate surface densities throughout their disks, when compared to local star forming samples. Comparing these measurements to predictions from star formation theory, we find very good agreements with the latest feedback-regulated star formation models. However, we find that theories which combine gravitational energy dissipation from radial gas transport with feedback over-estimate the observed molecular gas velocity dispersions.

==> Tables/LineRatiosSummary.tex <==
\begin{deluxetable*}{lccc}
\tablecaption{CO(4$-$3)/CO(3$-$2) Line Ratios Compiled from the Literature Compared to DYNAMO} 
\label{tab:lrs}
\tablewidth{700pt}
\tabletypesize{\scriptsize}
\tablehead{
    \colhead{Object(s)}        &
	\colhead{Line Ratio}       &
	\colhead{Reference}        &
	\colhead{Notes}
} 
\startdata
$z = 1.5$ MS Galaxies & 0.74 $\pm$ 0.26 & \citet{daddi15} & interpolated \\
G1700-MD94 one component model & $0.92 \pm 0.18$ & \citet{henriquez-brocal21} & interpolated \\
G1700-MD94 two component model & $0.77 \pm 0.15$ & \citet{henriquez-brocal21} & interpolated \\
ULIRGs low CO excitation & 1.08 & \citet{rosenberg15} & \\
ULIRGs mid CO excitation & 0.70 & \citet{rosenberg15} & \\
ULIRGs high CO excitation & 1.02 & \citet{rosenberg15} & \\
LIRGs & 0.49 $\pm$ 0.18 & \citet{papadopoulos12} & \\
ULIRGs & $1.32 \pm 0.26$ & \citet{kamenetzky16} & $log(L_{FIR}) = 12$ \\
non-(U)LIRGs & $0.24 \pm 0.0.05$ & \citet{kamenetzky16} & $log(L_{FIR}) = 10$ \\
C22-2 & 0.62 $\pm$ 0.13 & This work & \\
D13-5 & 0.57 $\pm$ 0.08 & This work & \\
G04-1 & 0.50 $\pm$ 0.08 & This work & \\
G14-1 & 0.71 $\pm$ 0.11 & This work & \\
G20-2 & 0.61 $\pm$ 0.07 & This work & \\
SDSS J013527.10-103938.6 & 0.44 $\pm$ 0.05 & This work \\
DYNAMO all & $0.54${\raisebox{0.5ex}{\tiny$^{+0.16}_{-0.15}$}} & This work & \\
\enddata
% \tablenotetext{\scriptsize{a}}{Values from \citet{green14}.} \tablenotetext{\scriptsize{b}}{Values from \citet{fisher17b}.} \tablenotetext{\scriptsize{c}}{Mean H$_{\alpha}$ extinction and $1\sigma$ scatter of all clump pixels from \citet{bassett17}.}
% \tablenotetext{\scriptsize{d}}{Median clump size for each galaxy, see \S\ref{subsec: clumpd_ID} for details on clump size measurements.}
\end{deluxetable*}

==> Tables/ObsTable.tex <==
\begin{deluxetable}{lccc}
\tablecaption{CO Data Cube Parameters} 
\label{tab:obs}
\tablewidth{700pt}
\tabletypesize{\scriptsize}
\tablehead{
% 	\colhead{Galaxy} 			           &
	\colhead{CO Trans.}                    &
	\colhead{Beam FWHM}                    &
	\colhead{rms Noise}                    &
	\colhead{{\sc casa} Cal.}      \\
% 	\colhead{}                             &
	\colhead{}                             &
	\colhead{(arcsec)}                     &
	\colhead{(mK)}                         &
	\colhead{}                             
} 
\startdata
\sidehead{DYNAMO C13-1}
$3-2$ & 1.07 & 11.5 & v5.1.1-5 \\
\hline
\sidehead{DYNAMO C22-2}
$3-2$ & 1.07 & 16.0 & v5.1.1-5 \\
$4-3$ & 0.81 & 12.5 & v5.1.1-5 \\
\hline
\sidehead{DYNAMO D13-5}
$3-2$ & 1.10 & 8.2 & v5.1.1-5 \\
$4-3$ & 0.79 & 12.1 & v5.1.1-5 \\
\hline
\sidehead{DYNAMO D15-3}
$4-3$ & 0.96 & 10.8 & v5.1.1-5 \\
\hline
\sidehead{DYNAMO G04-1}
$3-2$ & 0.42 & 29.1 & v5.6.1-8 \\
$4-3$ & 0.84 & 21.5 & v5.1.1-5 \\
\hline
\sidehead{DYNAMO G08-5}
$3-2$ & 0.40 & 32.4 & v5.6.1-8 \\
\hline
\sidehead{DYNAMO G14-1}
$3-2$ & 1.06 & 3.3 & v5.1.1-5 \\
$4-3$ & 0.85 & 6.3 & v5.1.1-5 \\
\hline
\sidehead{DYNAMO G20-2}
$3-2$ & 1.23 & 3.7 & v5.1.1-5 \\
$4-3$ & 0.86 & 4.8 & v5.1.1-5 \\
\hline
\sidehead{SDSS J013527.10-103938.6}
$3-2$ & 1.23 & 5.2 & v5.1.1-5 \\
$4-3$ & 0.86 & 4.5 & v5.1.1-5 \\
\enddata
% \tablenotetext{\scriptsize{a}}{Values from \citet{green14}.} \tablenotetext{\scriptsize{b}}{Values from \citet{fisher17b}.} \tablenotetext{\scriptsize{c}}{Mean H$_{\alpha}$ extinction and $1\sigma$ scatter of all clump pixels from \citet{bassett17}.}
% \tablenotetext{\scriptsize{d}}{Median clump size for each galaxy, see \S\ref{subsec: clumpd_ID} for details on clump size measurements.}
\end{deluxetable}
